Constrained Upper Confidence Reinforcement Learning

Constrained Markov Decision Processes are a class of stochastic decision problems in which the decision maker must select a policy that satisfies auxiliary cost constraints. This paper extends upper confidence reinforcement learning for settings in which the reward function and the constraints, described by cost functions, are unknown a priori but the transition kernel is known. Such a setting is well-motivated by a number of applications including exploration of unknown, potentially unsafe, environments. We present an algorithm C-UCRL and show that it achieves sub-linear regret ($ O(T^{\frac{3}{4}}\sqrt{\log(T/\delta)})$) with respect to the reward while satisfying the constraints even while learning with probability $1-\delta$. Illustrative examples are provided.

==> algo_old.tex <==

%\section{Algorithm}



As noted in the introduction, since the reward and constraint cost functions are unknown, motivated by UCRL, we introduce the constrained UCRL algorithm given in Algorithm~\ref{alg:safeUCRL}. In general, the C-UCRL algorithm follows a principle of ``optimism in the face of reward uncertainty; pessimism in the face of cost uncertainty." That is, it defines confidence intervals for the reward and cost of each state-action pair given the observations so far, and solves for the optimistic policy that satisfies the constraints.
More specifically, in C-UCRL, given the current confidence interval estimates, we use a robust linear program \citep{luenberger1984linear} formulation to find a policy using the confidence intervals as determined at the current iteration. In particular, in episode $k$, we define 
estimates of the reward and costs by
 \[\hat{r}_k(s, a) = \textstyle\frac{R_k(s, a)}{\max \{1, N_k(s, a)\}}\  \text{and}\ \hat{c}_{i,k}(s, a) = \frac{C_{i, k}(s, a)}{\max \{1, N_k(s, a)\}},\]
 respectively, where $N_k(s,a)$, $R_k(s,a)$, and $C_{i,k}(s,a)$ are the  state-action count, and cumulative reward and costs, respectively, as defined in Algorithm~\ref{alg:safeUCRL}.
 Using these estimates, we define
\begin{equation}
\tilde{r}_k(s, a)  = \textstyle\min \big\{ \hat{r}_k(s,a) + \big(\frac{\log (S A (m+1) \pi^2 t_k^3 / 3 \delta)}{2 \max \{1, N_k(s,a)\}}\big)^{1/2}, 1 \big\} 
\label{eq:tilder}
\end{equation}
and
\begin{equation}
\tilde{c}_{i,k}(s, a)  =\textstyle \min \big\{ \hat{c}_{i,k}(s,a) + \big(\frac{\log (S A (m+1) \pi^2 t_k^3 / 3 \delta)}{2 \max \{1, N_k(s,a)\}}\big)^{1/2}, 1 \big\},
\label{eq:tildec}\end{equation}
and solve the following robust linear program:
\begin{equation}
\max_{y} \{ \ \tilde{r}_k^\top y \ | \ I_o y = P y, \ \mathbf{1}^\top y = 1, \ y \ge 0, \ \tilde{c}_k^\top y \le d\} \tag{RLP}\label{eq:RLP}
\end{equation}

$N_k(s,a)$ the total number of times $(s,a)$ has been visited prior to episode $k$. $R_k(s,a)$ and $C_{i,k}(s,a)$ are the observed accumulated rewards and cost prior to episode $k$.
%\textcolor{red}{Need to say somethign about how things like $N_k$, $R_k$, etc are initilized either here or in the algorithm block.}

As in \eqref{eq:tilder} and \eqref{eq:tildec}, the confidence intervals of reward and cost depend on the visit times of that state-action pair.
%\textcolor{red}{this is super hand wavy and I am not sure i know what you mean by 'after enough exploration'}
%\lily{you are going to have to formalize this or provide some commentary on what the implication of this assumption is... how strong is it for example? how would you verify it? how much exploration do you need?}
To trade-off between exploration and exploitation, we assume we are given a safe baseline policy as a input of C-UCRL. It is common to assume a initial safe policy before learning procedure \citep{achiam2017constrained} and without loss of generality, we assume under such policy, the Markov chain resulting from the CMDP is irreducible and aperiodic \citep{bhatnagar2009natural}. This baseline policy could be obtained by some prior information about which states are safe to start the conservative exploration. %\textcolor{red}{can you at least put some discussion of how you might obtain a baseline?} 
We execute the baseline policy in the early learning stage to build estimation of reward and cost by \eqref{eq:tilder} and \eqref{eq:tildec} until there is a feasible solution to \eqref{eq:RLP}. Then, we recover the policy $\tilde{\pi}_k$ from the occupation measure $\tilde{y}_k$ obtained from \eqref{eq:RLP}. In each episode of C-UCRL algorithm, we execute the baseline policy for fixed  number steps $h$ and execute $\tilde{\pi}_k$ for a linearly increasing (in the number of epochs) number of steps $(k-1)h$.


%\lily{You will have to comment on this too. Why is it reasonable that you have access to a baseline policy and how would you design such a policy?} 

\input{algorithm.tex}



==> analysis_old.tex <==
\section{Analysis}
\label{sec:analysis}

In this section, we summarize our analysis results. We first show that C-UCRL has guarantees on constraint satisfaction during learning. Then, we provide regret analysis with respect to the reward, showing that the regret is sub-linear. To capture constraint satisfaction, we leverage the notion of $\delta$-safety. 

\begin{definition}[$\delta$-safe]
	An algorithm is $\delta$-safe if, with probability at least $1-\delta$, for all time steps $t$, the policy executed by the algorithm satisfies
$C_i(\pi_t) \le d_i$, $\forall i \in [m]$.
\end{definition}

\begin{lemma} \label{lemma:unionbound}
	With probability at least $1-\delta$, for every state-action pair $(s,a)$, cost $c_i$ and episode $k$,
	C-UCRL satisfies the following:
	\begin{align}
	| \hat{r}_k(s,a) - \bar{r}(s,a)| & \le \textstyle\big(\frac{\log (S A (m+1) \pi^2 t_k^3 / 3 \delta)}{2 \max \{1, N_k(s,a)\}}\big)^{1/2}, \\
	|\hat{c}_{i,k}(s,a) - \bar{c}_i(s,a)| & \textstyle\le \big(\frac{\log (S A (m+1) \pi^2 t_k^3 / 3 \delta)}{2 \max \{1, N_k(s,a)\}}\big)^{1/2}
	\end{align}
\end{lemma}

\begin{proof}
	Consider a fixed state-action pair $(s,a)$ and assume some given number of visits $n>0$ in $(s,a)$ before episode $k$. For both the reward and costs, we observe real-valued, independent identically distributed (iid) random variables supported on $[0,1]$. For such settings, applying Hoeffding's inequality we get the following bound on the deviation between the true mean $\bar{r}(s,a)$ and the empirical mean $\hat{r}_{k}(s,a)$ from $n$ iid samples:
	\begin{equation}
	\Pr \left\{ |\hat{r}_{k}(s,a) - \bar{r}(s,a)| \ge \epsilon_r \right\} \le 2 \exp (-2 n \epsilon_r^2)
	\end{equation}
	Setting
	$\epsilon_r = \big(\log (S A (m+1) \pi^2 t_k^3 / 3 \delta)/(2 n)\big)^{1/2}$,
	we get for each state-action pair $(s,a)$
	\begin{equation}
	\Pr \left\{ |\hat{r}_{k}(s,a) - \bar{r}(s,a)| \ge \epsilon_r \right\}  
	%= \Pr \Big\{ |\hat{r}_{k}(s,a) - \bar{r}(s,a)| \ge \sqrt{\frac{\log (S A (m+1) \pi^2 t_k^3 / 3 \delta)}{2 n}} \Big\} \\
%	& \le 2 \exp \left( -2 n \frac{\log (S A (m+1) \pi^2 t_k^3 / 3 \delta)}{2 n} \right) \\
	 = 6 \delta/(S A (m+1) \pi^2 t_k^3).
	\end{equation}
	Similarly, for each state-action pair $(s,a)$ and cost $c_i$,
	%\lily{Just to be clear here, you are picking the same $\epsilon_r$ as you did with the reward right? if so maybe we can just make that clear and drop the r subscript on $\epsilon$.}
	\begin{equation}
	\Pr \{ |\hat{c}_{i,k}(s,a) - \bar{c}_i(s,a)| \ge \epsilon_r\}
	%\sqrt{\frac{\log (S A (m+1) \pi^2 t_k^3 / 3 \delta)}{2 n}} \right\} 
	\le 6 \delta/(S A (m+1) \pi^2 t_k^3).
	\end{equation}
	Note that when there has not been any observations for a state $s$ and action $a$, the confidence interval trivially holds with probability one for both reward and costs. Hence, union bounds over all state-action pairs $(s,a)$, cost indexed by $i \in \{1, \dots, m\}$, all possible values of $n = 1,\dots, t_k$ and $t_k=1, \dots, \infty$ gives us the following bounds:
	\begin{equation*}
	    	\textstyle \Pr \big\{ \cup_{t_k = 1}^{\infty} \cup_{n = 1}^{t_k} \cup_{s,a} \big\{ |\hat{r}_{k}(s,a) - \bar{r}(s,a)| \ge \epsilon_r %\sqrt{\frac{\log (S A (m+1) \pi^2 t_k^3 / 3 \delta)}{2 n}} 
	    	\big\} \big\} \textstyle\le \sum_{t_k=1}^{\infty} \sum_{n = 1}^{t_k} \sum_{s,a} \frac{6 \delta}{S A (m+1) \pi^2 t_k^3} = \frac{\delta}{m+1}
	\end{equation*}
	%\begin{align}
%	& \Pr \left\{ \bigcup_{t_k = 1}^{\infty} \bigcup_{n = 1}^{t_k} \bigcup_{s,a} \left\{ |\hat{r}_{k}(s,a) - \bar{r}(s,a)| \ge \sqrt{\frac{\log (S A (m+1) \pi^2 t_k^3 / 3 \delta)}{2 n}} \right\} \right\} \\
%	&\le \sum_{t_k=1}^{\infty} \sum_{n = 1}^{t_k} \sum_{s,a} \frac{6 \delta}{S A (m+1) \pi^2 t_k^3} = \frac{\delta}{m+1}
%	\end{align}
	and
	\begin{equation*}
	    	 \textstyle\Pr \big\{ \cup_{t_k = 1}^{\infty} \cup_{n = 1}^{t_k} \cup_{s,a,i} \big\{ |\hat{c}_{i,k}(s,a) - \bar{c}_i(s,a)| \ge \epsilon_r %\sqrt{\frac{\log (S A (m+1) \pi^2 t_k^3 / 3 \delta)}{2 n}} 
	    	 \big\} \big\} 
	    	\le \sum_{t_k=1}^{\infty} \sum_{n = 1}^{t_k} \sum_{s,a,i} \frac{6 \delta}{S A (m+1) \pi^2 t_k^3} = \frac{m\delta}{m+1}
	\end{equation*}
%	\begin{align}
%	& \Pr \left\{ \bigcup_{t_k = 1}^{\infty} \bigcup_{n = 1}^{t_k} \bigcup_{s,a,i} \left\{ |\hat{c}_{i,k}(s,a) - \bar{c}_i(s,a)| \ge \sqrt{\frac{\log (S A (m+1) \pi^2 t_k^3 / 3 \delta)}{2 n}} \right\} \right\} \\
%	&\le \sum_{t_k=1}^{\infty} \sum_{n = 1}^{t_k} \sum_{s,a,i} \frac{6 \delta}{S A (m+1) \pi^2 t_k^3} = \frac{m\delta}{m+1}
%	\end{align}
	where we use the fact that $\sum_{n=1}^\infty \frac{1}{n^2} = \frac{\pi^2}{6}$. Summing these error probabilities for the reward and costs, we obtain the union bound given by
	\begin{equation*}
	    \Pr \{ 
	|\hat{r}_{k}(s,a) - \bar{r}(s,a)|  \ge \epsilon_r %\sqrt{\frac{\log (S A (m+1) \pi^2 t_k^3 / 3 \delta)}{2 \max \{1, N_k(s,a)\}}}, \\
	\land
	|\hat{c}_{i,k}(s,a) - \bar{c}_i(s,a)|  \ge \epsilon_r\} %\sqrt{\frac{\log (S A (m+1) \pi^2 t_k^3 / 3 \delta)}{2 \max \{1, N_k(s,a)\}}}
	%\end{aligned} \right\} 
	\le \delta.
	\end{equation*}
	%\begin{equation}
	%\Pr \left\{ \begin{aligned}
	%|\hat{r}_{k}(s,a) - \bar{r}(s,a)| & \ge %\sqrt{\frac{\log (S A (m+1) \pi^2 t_k^3 / 3 %\delta)}{2 \max \{1, N_k(s,a)\}}}, \\
	%|\hat{c}_{i,k}(s,a) - \bar{c}_i(s,a)| & \ge %\sqrt{\frac{\log (S A (m+1) \pi^2 t_k^3 / 3 %\delta)}{2 \max \{1, N_k(s,a)\}}}
	%\end{aligned} \right\} \le \delta
	%\end{equation}
	%\lily{what does this notation mean? you are trying to say the probability of the event that the reward gap is above some threshold AND the cost gap right? I am going to change it}
\end{proof}

Given that, for each episode, we can bound the gaps between the estimated reward (respectively, costs) and the mean reward (respectively, mean costs), with probability $1-\delta$, we can provide an assurance on C-UCRL being $\delta$-safe.
\begin{theorem}
C-UCRL is $\delta$-safe. 
\label{thm:deltasafe}
\end{theorem}

\begin{proof}
	According to Lemma~\ref{lemma:unionbound}, with probability at least $1-\delta$, $\bar{c}_i(s, a) \le \tilde{c}_{i,k}(s,a)$. The occupation measure $\tilde{y}_k$ obtained at each episode via \eqref{eq:RLP}
	%solved by the robust linear program defined in \textcolor{red}{xxx}, 
	satisfies $\sum_{s,a} \tilde{c}_{i,k}(s,a) \tilde{y}_k(s,a) \le d_i$.
	%\textcolor{red}{and thus,} 
Hence,	 $C_i(\tilde{\pi}_k) = \sum_{s,a} \bar{c}_{i}(s,a) \tilde{y}_k(s,a) \le d_i$ with probability $1-\delta$.
\end{proof}

Given that we have shown that C-UCRL is $\delta$-safe,  we now analyze the reward regret. In episode $k$ of C-UCRL, we execute a baseline policy $\pi_0$ for $h$ times and policy $\tilde{\pi}_k$ for $(k-1)h$ times. The pseudo-regret of episode $k$ is given by
\begin{equation*}
\Delta_k  = h [J(\bar{\pi}) - J(\pi_0)] + (k-1)h [J(\bar{\pi}) - J(\tilde{\pi}_k)] = h \bar{r}^\top (\bar{y} - y_0) + (k-1)h \bar{r}^\top (\bar{y} - \tilde{y}_k).
\end{equation*}

We first upper bound the per-step pseudo-regret of executing policy $\tilde{\pi}_k$, $\bar{r}^\top (\bar{y} - \tilde{y}_k)$, where the first term is the expected average reward under the optimal policy $\bar{\pi}$ and the second term is the sub-optimal expected average reward under policy $\tilde{\pi}_k$.

Define the following two linear programs:
\begin{align}
    &\textstyle\max_y \{ r^\top y | Ay=0, \mathbf{1}^\top y = 1, y \ge 0, c^\top y \le d \}    \label{eq:y1}\\
    &\textstyle\max_y \{ (r+\epsilon_r)^\top y | Ay=0, \mathbf{1}^\top y = 1, y \ge 0, (c+\epsilon_c)^\top y \le d \}.
    \label{eq:y2}
\end{align}
where  
	$0 \le r \le \mathbf{1}$, $0 \le c \le \mathbf{1}$, $\epsilon_r \ge 0$, and $\epsilon_c \ge 0$ hold element wise. 

\begin{lemma} 
	%	\textcolor{red}{I dont think you should use $y_n$ (same for others) since you are using subscript $k$ for time index on some other $y$ variables. That makes it confusing.} 
	Assuming the domains of \eqref{eq:y1} and \eqref{eq:y2} are not empty, let $y_1$ and $y_2$ be  solutions for each of the problems, respectively. %\textcolor{red}{Why is this a reasonable assumption? Perhaps a footnote explaing that...} 
	%\lily{It should be clear that these things are true already by the previous assumptions so we should just state in the previous section that throughout we assume the reward and costs are supported on $[0,1]$ and I assume these inequalities are elementwise?}. If there exists \lily{Is there an $r^\top $ missing in this $y_0$ problem?} 
	If, for some constant $\alpha > 0$ and $\beta > 0$, there exist $y_0 \in \{y | Ay = 0, \mathbf{1}^\top y = 1, y \ge 0, (c+\epsilon_c)^\top y \le d \}$ such that $r^\top (y_1-y_0) = \alpha >0$ and $c^\top (y_1-y_0) = \beta >0$, then
	%\lily{we need to justify this assumption that $\alpha, \beta>0$. If we can do that I buy your proof for this lemma}, then
	\begin{equation}
	r^\top (y_1 - y_2) \le \frac{2\alpha}{\beta} \| \epsilon_c \|_1 + \|\epsilon_r\|_1.
	\end{equation}
	%\lily{You have not defined $\epsilon_c$. I assume that $\epsilon_c=\epsilon_r$ by the previous Lemma?}
	\label{lemma:pseudoregret}
\end{lemma}

\begin{proof}
	Let $y_3 = \arg\max_y \{ r^\top y | Ay=0, \mathbf{1}^\top y = 1, y \ge 0, (c+\epsilon_c)^\top y \le d \}$.
	We first find the upper bound of $r^\top (y_1- y_3)$ where we note that $y_3$ and $y_1$ are the solutions of same linear program over different domains. Since the domain of $y_3$ is smaller than $y_1$, we know that $r^\top (y_1- y_3) \ge 0$. 
	First, consider the trivial case that $y_1$ satisfies $(c+ \epsilon_c)^\top y_1 \le d$. In this case, $y_1 = y_3$ and $r^\top (y_1- y_3) = 0$. Now we only consider the case such that $(c+ \epsilon_c)^\top y_1 > d$. Note that $(c+ \epsilon_c)^\top y_0 \le d$. Hence, there exist $\gamma \in [0,1)$ such that $y_4 = y_0 + \gamma (y_1-y_0)$ and $(c+\epsilon_c)^\top y_4 = d$, (i.e. $\gamma = \frac{d - (c+\epsilon_c)^\top y_0}{(c+\epsilon_c)^\top (y_1-y_0)}$). Further, we have $y_1-y_4=y_1 - y_0 - \gamma(y_1-y_0)=(1-\gamma)(y_1-y_0)$, thus $c^\top  (y_1-y_4)= (1-\gamma) \beta >0$
	and 
	\begin{align}
	c^\top (y_1-y_4) & = (c+\epsilon_c)^\top (y_1-y_4) - \epsilon_c^\top (y_1-y_4) = c^\top y_1 + \epsilon_c^\top  y_1 -d - \epsilon_c^\top (y_1-y_4) \\
	& \le d-d + \epsilon_c^\top y_1 -  \epsilon_c^\top (y_1-y_4) \le \| \epsilon_c \|_1 \|y_1\|_\infty + \| \epsilon_c \|_1 \| y_1-y_4 \|_\infty = 2\|\epsilon_c\|_1
	\end{align}
Combine with
\begin{equation}
\frac{r^\top (y_1-y_4)}{c^\top  (y_1-y_4)} =  \frac{r^\top (y_1-y_0)}{c^\top  (y_1-y_0)} = \frac{\alpha}{\beta}
\end{equation}
we have $0 < r^\top  (y_1-y_4) \le 2 \frac{\alpha}{\beta} \|\epsilon_c\|_1$. According to the convexity of the domain, we know that $y_4$ must be within the domain $y_4 \in \{y | Ay=0, \mathbf{1}^\top  y = 1, y\ge 0, (c+\epsilon_c)^\top y \le d \}$. Because of the optimality $r^\top  y_3 \ge r^\top  y_4$, we get $r^\top  (y_1-y_3) \le 2 \frac{\alpha}{\beta} \|\epsilon_c\|_1$.




	
	
	
	%We also only consider the case that $c^\top  y_1 = d$ since otherwise the constraint is not active, and hence, would not be considered in the problem. We have that
	%$(c + \epsilon_c)^\top  y_1  = c^\top  y_1 + \epsilon_c^\top  y_1  \le d + \| \epsilon_c \|_1 \|y_1\|_\infty  \le d + \| \epsilon_c \|_1$.
	%We know that the optimal solution will lie on the vertices of the domain such that $(c+ \epsilon_c)^\top  y_3 = d$; hence, 
	%$(c + \epsilon_c)^\top  (y_1 - y_3) \le \| \epsilon_c \|_1$.
	%Further, we have \lily{ should this be $0\leq c^\top (y_1-y_3)$? $\epsilon_c\geq0$... Even if $\epsilon_c>0$ if this inequality is elementwise I do not think you can guarantee that $0<c^\top(y_1-y_3)$ because you could have zero probability for some state-action pairs... is $c^\top y$ a scalar? I thought $c$ was a matrix with all the constraints $c_i$ stacked up and $d$ was a vector... is $c>0$? If this is not the case I dont see how you get strict in equality... for example, if $c=[1\ 0\ 0\ 0\ 0]$ and $y=[0\ 1/2\ 1/4\ 1/4]^\top$, then $c^\top y=0$ so even if $y_1\neq y_3$ it could still be the case that $c^\top (y_1-y_3)=0$. Maybe you can assume that $c>0$ and argue that $y_1-y_3\neq 0$? or can you argue this without the fraction so that there is no divide by zero problem? }
	%\textcolor{blue}{Because we have $c^\top y_1 = d$ and $(c+\epsilon_c)^\top  y_3 = d$, thus $c^\top  (y_1 - y_3) = c^\top  y_1 - (c+\epsilon_c)^\top  y_3 + \epsilon_c y_3 = d-d + \epsilon_c y_3 = \epsilon_c y_3$. If we assume $\epsilon_c > 0$, then $\epsilon_c y_3 > 0$ because $\mathbf{1}^\top  y_3 = 1$.}
	%\begin{equation*}
	%	0 <c^\top  (y_1 - y_3)  = (c+\epsilon_c)^\top  (y_1-y_3) - \epsilon_c^\top  (y_1-y_3)  \le  \| \epsilon_c \|_1 + \| \epsilon_c \|_1 \| y_1-y_3\|_\infty  \le 2  \| \epsilon_c \|_1
	%\end{equation*}
%Let $y_4 = y_0 + \gamma (y_1 - y_0)$ such that $(c+ \epsilon_c)^\top  y_4 = d$. Because of the convexity of the domain, $y_4$ must be within the domain, $y_4 \in \{y | Ay=0, \mathbf{1}^\top  y = 1, y\ge 0, (c+\epsilon_c)^\top y \le d \}$. Similarly, we have $0 < c^\top (y_1-y_4) \le 2 \|\epsilon_c\|_1$. Additionally, from
%\begin{equation}
%\frac{r^\top  (y_1-y_4)}{c^\top  (y_1-y_4)} =  \frac{r^\top (y_1-y_0)}{c^\top  (y_1-y_0)} = \frac{\alpha}{\beta}
%\end{equation}\lily{have you shown $c^\top(y_1-y_0)!=0$? Oh you are assuming this is true... hmm we justify why or when this is possible...}
%we have $r^\top  (y_1 - y_4) \le 2 \frac{\alpha}{\beta} \|\epsilon_c\|_1$. According to optimality, we know that $r^\top  y_3 \ge r^\top  y_4$. Thus, $r^\top  (y_1 - y_3) \le 2 \frac{\alpha}{\beta} \|\epsilon_c\|_1$.
	
	
	%Here we need the assumption that, $\forall \Delta y \in null \begin{pmatrix}
	%A \\
	%\mathbf{1}^\top  
	%\end{pmatrix}, \gamma \in [0, 1]$
	%\begin{equation}
	%|(c+ \gamma \epsilon_c)^\top  \Delta y| \ge const \cdot \| \Delta y\|_2
	%\end{equation}
	%where $\mathcal{N} = null \begin{pmatrix}
	%A \\
	%\mathbf{1}^\top  
	%\end{pmatrix}$.
	
	%Let $\mathcal{N} = null \begin{pmatrix}
	%A \\
	%\mathbf{1}^\top  
	%\end{pmatrix}$, if for all $\Delta y \in \mathcal{N}$ and $\gamma \in [0, 1]$, $(c + \gamma \epsilon_c)^\top  \Delta y %\ne 0$
	%\begin{equation}
	%|(c+ \epsilon_c)^\top  \Delta y| \ge const \cdot \| \Delta y\|_2
	%\end{equation}
	
	%Thus we have 
	%\begin{equation}
	%r^\top  (y_1 - y_3) \le |y_1 - y_3| \le const \cdot |\epsilon_c|
	%\end{equation}
	%The first inequality is because $ 0\le r \le \mathbf{1}$. 
	
	
	%Define matrix $A' =  \begin{pmatrix}
	%A \\
	%\mathbf{1}^\top  
	%\end{pmatrix}$ and denote $\mathcal{N}(A')$ as the null space of matrix $A'$. Note that $y_1 - y_3 \in \mathcal{N}(A')$. We make assumption that for all $\gamma_i \in [0,1]$, $c + \gamma \odot \epsilon_c \in \mathcal{N}(A')$, where $\odot$ denotes element wise product.
	
	%Now we project the convex set $\{y | Ay = 0, \mathbf{1}^\top  y = 1, y \ge 0 \}$ on to the plane expanded by vector $c+ \epsilon_c$ and $r$. The projected set is a convex polygon. The projected $y_3$ is on the vertex of the polygon. Assume it is on the boundary of $(c+ \epsilon_c)^\top y \le d$ and $a^\top  y \le b$, as $(c+ \epsilon_c)^\top y_3 = d$ and $a^\top y_3=b$. Note that this $a$ vector is in the plane of $c+ \epsilon_c$ and $r$, $a = \alpha (c+\epsilon_c) + \beta r$. Because $(c+ \epsilon_c) \in \mathcal{N}(A')$, the boundary of $a$ is not parallel to the boundary of $c+ \epsilon_c$, $a \nparallel (c+ \epsilon_c)$, $\beta \ne 0$. 
	
	%For the projected $y_1$, as shown before we have, $d < (c+\epsilon_c)^\top  y_1 \le d + \|\epsilon_c\|$. The projected polygon is convex so it is in the boundary, $a^\top  y_1 \le b$. Also we know that $r^\top  (y_1 - y_3) \ge 0$. Thus $r^\top (y_1 - y_3) \le const \cdot \|\epsilon_c\|$.
	
	
	Now that we have the bound on $r^\top (y_1 - y_3)$ and we try to further bound $r^\top  (y_3 - y_2)$. Note that $y_3$ and $y_2$ are the solutions of two linear programs with different objectives but the same domain. According to optimality of the solutions, we know that $r^\top  y_3 \ge r^\top  y_2$ and $(r+ \epsilon_r)^\top  y_2 \ge (r + \epsilon_r)^\top  y_3$. Combine these facts, we have that
	\begin{equation}
	0 \le r^\top  (y_3 - y_2) \le \epsilon_r^\top  (y_2 - y_3) \le \|\epsilon_r\|_1 \|y_2 - y_3\|_\infty \le \|\epsilon_r\|_1
	\end{equation}
	
	Now, combining the bounds on $r^\top  (y_3 - y_2)$ and $r^\top  (y_1 - y_3)$, we have that
	\begin{equation}
	r^\top  (y_1 - y_2) = r^\top  (y_1 - y_3) + r^\top  (y_3 - y_2) \le \frac{2\alpha}{\beta} \| \epsilon_c \|_1 + \|\epsilon_r\|_1 %\le \max\{\frac{2\alpha}{\beta}, 1\} \cdot (\|\epsilon_c\|_1 + \|\epsilon_r\|_1)
	\end{equation}
	%where $const = \max\{\frac{2\alpha}{\beta}, 1\}$.
	%\lily{As I have mentioned before. i dont think you should use 'const'. you define this constant. there is no reason not to plug it in here. it looks bad asthetically...}
\end{proof}

We can use Lemma~\ref{lemma:pseudoregret} to prove the following proposition.

\begin{proposition}[Pseudo-regret Bound.] \label{thm:pseudoregret}
	Denote $\mathcal{Y} = \{y | (I_o - P)y = 0, \mathbf{1}^\top y = 1, y \ge 0 \}$. If there exists $y_0 \in \mathcal{Y}$ such that $\bar{r}^\top (\bar{y}-y_0) = \alpha >0, \bar{c}^\top(\bar{y}-y_0) = \beta >0$, then with probability at least $1-\delta$,
	\begin{equation}
	\bar{r}^\top (\bar{y} - \tilde{y}_k) \le 2 (\frac{2\alpha m}{\beta} + 1)  \sum_{s, a} \sqrt{\frac{\log (S A (m+1) \pi^2 t_k^3 / 3 \delta)}{2 \max \{1, N_k(s,a)\}}}.
	\end{equation}
\end{proposition}

\begin{proof}
	By definition $\bar{y} = \arg\max_y \{ \bar{r} ^\top y | (I_o - P) y=0, \mathbf{1}^\top y = 1, y \ge 0, \bar{c}_i^\top y \le d_i, i \in [1, \dots, m]\}$ and $\tilde{y}_k = \arg\max_y \{ \tilde{r}_k^\top y | (I_o - P) y=0, \mathbf{1}^\top y = 1, y \ge 0, \tilde{c}_{i,k}^\top y \le d_i, i \in [1, \dots, m]\}$. Define a sequence of subproblem by adding one constraint at a time
	\begin{equation}
	\begin{aligned}
	y^{(1)} & = \arg\max_y \{ \bar{r} ^\top y | (I_o - P) y=0, \mathbf{1}^\top y = 1, y \ge 0, \tilde{c}_{1,k}^\top y \le d_1, \bar{c}_i^\top y \le d_i, i \in [2, \dots, m]\} \\
	y^{(2)} & = \arg\max_y \{ \bar{r} ^\top y | (I_o - P) y=0, \mathbf{1}^\top y = 1, y \ge 0, \tilde{c}_{1,k}^\top y \le d_1, \tilde{c}_{2,k}^\top y \le d_2, \bar{c}_i^\top y \le d_i, i \in [3, \dots, m]\}  \\
	& \ \ \vdots \\
	y^{(m)} & = \arg\max_y \{ \bar{r} ^\top y | (I_o - P) y=0, \mathbf{1}^\top y = 1, y \ge 0, \tilde{c}_{i,k}^\top y \le d_i,  i \in [1, \dots, m]\}
	\end{aligned}
	\end{equation}
	Using the same proof in Lemma~\ref{lemma:pseudoregret}, we obtain the bounds for $\bar{r}^\top (\bar{y} - y^{(1)}), \bar{r}^\top (y^{(1)} - y^{(2)}), \dots, \bar{r}^\top (y^{(m-1)} - y^{(m)}), \bar{r}^\top (y^{(m)} - \tilde{y}_{k})$. Combining the bounds and the fact that $\epsilon_r(s,a) = \tilde{r}_k(s,a) - \bar{r}(s,a) \le 2 \sqrt{\frac{\log (S A (m+1) \pi^2 t_k^3 / 3 \delta)}{2 \max \{1, N_k(s,a)\}}}, \epsilon_c(s,a) = \tilde{c}_{i,k}(s,a) - \bar{c}_i(s,a) \le 2 \sqrt{\frac{\log (S A (m+1) \pi^2 t_k^3 / 3 \delta)}{2 \max \{1, N_k(s,a)\}}}$, we have
	\begin{align}
	\bar{r}^\top (\bar{y} - \tilde{y}_{k}) & = \bar{r}^\top (\bar{y} - y^{(1)}) + \dots + \bar{r}^\top (y^{(m)} - \tilde{y}_{k}) \le m \frac{2\alpha}{\beta} \| \tilde{c}_k - \bar{c} \|_1 + \| \tilde{r}_k - \bar{r} \|_1 \\
	&\le 2 (\frac{2\alpha m}{\beta} + 1) \sum_{s,a} \sqrt{\frac{\log (S A (m+1) \pi^2 t_k^3 / 3 \delta)}{2 \max \{1, N_k(s,a)\}}}
	\end{align}
	
\end{proof}


Note that according to Proposition~\ref{thm:pseudoregret}, with probability at least $1-\delta$,
%if our confidence intervals of reward and costs hold, $|\hat{r}_k(s,a) - \bar{r}(s,a)| \le \sqrt{\frac{\log (S A (m+1) \pi^2 t_k^3 / 3 \delta)}{2 \max \{1, N_k(s,a)\}}}, \forall s, a$ and $|\hat{c}_{i,k}(s,a) - \bar{c}_i(s,a)| \le \sqrt{\frac{\log (S A (m+1) \pi^2 t_k^3 / 3 \delta)}{2 \max \{1, N_k(s,a)\}}}, \forall s,a,i$, 
the per-step pseudo-regret of executing policy $\tilde{\pi}_k$ depends on the confidence intervals of reward and costs of all state-action pairs. This is intuitive since in order for the policy $\tilde{\pi}_k$ to be close to the optimal policy $\bar{\pi}$, we need to have good approximations of the reward and costs for all state-action pairs. To ensure this, we need to constantly explore the CMDP so that $N_k(s,a)$ is not `too small' for any state-action pair. Since the Markov chain resulting from the baseline policy is irreducible and aperiodic, the steady state occupation measure $y_0(s,a)$ corresponding to the baseline policy $\pi_0(a|s)$ has the property that $y_0(s,a) > 0, \forall s, a$.
%Thus, in C-UCRL algorithm, we use the irreducible and aperiodic baseline policy to explore the CMDP for constant a mount of time in each episode. 
%Assume that there exists a safe baseline policy $\pi_0(a|s)$ and the corresponding steady state $y_0(s,a)$ of baseline policy $\pi_0(a|s)$ such that $y_0(s,a) > 0, \forall s, a$. 
Due to this universal exploration demand, we execute the baseline policy $\pi_0$ for a constant number of times in each linear increasing episode in the C-UCRL algorithm.

To have a upper bound on the regret derived in Proposition~\ref{thm:pseudoregret}, we need to have a lower bounds on $N_k(s,a)$. Given our assumptions on the baseline policy as discussed above, define $\rho>0$ such that $y_0(s,a) \ge \rho > 0$  for all state-action pairs $(s,a)\in \mathcal{S}\times\mathcal{A}$.
The following lemma gives a lower bound on the number of times each state-action pair is visited in episode $k$.
%By repetitively executing the baseline policy for exploration, we obtain a lower bound on the visit times for each state-action pair in the following lemma.

\begin{lemma}  \label{lemma:visitcount}
	With probability at least $1-\delta$, for every state-action pair $(s,a)$ and episode $k$,
	\begin{equation}
\textstyle	N_k(s,a) \ge (k-1) \rho h - (k-1) \sqrt{72\xi \rho h \log\big(\frac{\varphi \cdot SAK}{\delta}\big)}
	\end{equation}
	where $\xi$ the the mixing time of the Markov chain induced by policy $\pi_0$ and $\varphi$ is a constant of inter product kernel of initial state-action distribution and steady state-action distribution.
\end{lemma}
\begin{proof}
	Consider the exploration phase (when the baseline policy $\pi_0$ is executed) of the $k$-th episode in Algorithm~\ref{alg:safeUCRL}. Consider a fixed state-action pair $(s,a)$, let $X_1, \dots, X_h$ be the indicator variables of whether state-action pair $(s,a)$ has be selected at each step. Let $X = \sum_{i=1}^hX_i$ and thus $\mathbb{E}[X] = y_0(s,a)h$. \citep[Theorem 3]{chung2012chernoff} gives 
	\begin{equation}
	\Pr \{ \mathbb{E}[X] - X \ge \epsilon y_0(s,a) h \} \le \varphi  \cdot \exp(-\frac{\epsilon^2 y_0(s,a) h}{72 \xi})
	\end{equation}
	Set
	\begin{equation}
	\epsilon = \sqrt{\frac{72\xi}{y_0(s,a)h} \log(\frac{\varphi \cdot SAK}{\delta})}
	\end{equation}
	this bound becomes
	\begin{equation}
	\Pr \left\{ X \le y_0(s,a)h - \sqrt{72\xi y_0(s,a)h \log(\frac{\varphi \cdot SAK}{\delta})} \right\} \le \frac{\delta}{SAK}
	\end{equation}
	Using the assumption that $y_0(s,a) \ge \rho > 0, \forall (s,a)$, we have the union bound over all state-action pair $(s,a)$ and episode $k=1, \dots, K$
	\begin{equation}
	\Pr \left\{ \bigcup_{(s,a), k} \left\{ X \le \rho h - \sqrt{72\xi \rho h \log(\frac{\varphi \cdot SAK}{\delta})} \right\} \right\} \le \sum_{s,a,k} \frac{\delta}{SAK} = \delta
	\end{equation}
	
	Simply summing over the first $k$ episodes, we have
	\begin{equation}
	N_k(s,a) \ge (k-1) \rho h - (k-1) \sqrt{72\xi \rho h \log(\frac{\varphi \cdot SAK}{\delta})}
	\end{equation}
	holds with probability at least $1-\delta$.
\end{proof}

Now we combine Proposition~\ref{thm:pseudoregret} and Lemma~\ref{lemma:visitcount} and sum over $K$ episode to obtaing the total regret bound for C-UCRL.

\begin{theorem}
	Under the assumptions of Proposition~\ref{thm:pseudoregret}, with probability at least $1-\delta$, C-UCRL has total pseudo-regret 
	\begin{equation}
	\Delta(T) = O(T^{\frac{3}{4}}\sqrt{\log(T/\delta)})
	\end{equation}
	\label{thm:regret}
\end{theorem}

\begin{proof}
	According to Claim~\ref{thm:pseudoregret}, the total regret of $K$ episode is 
	\begin{align}
		\sum_{k=1}^K \Delta_k & = \sum_{k=1}^K h \bar{r}^\top  (\bar{y} - y_0) + (k-1)h \bar{r}^\top  (\bar{y} - \tilde{y}_k) \\
		& = h K \bar{r}^\top  (\bar{y} - y_0) + h \sum_{k=2}^K (k-1) \bar{r}^\top  (\bar{y} - \tilde{y}_k) \\
		& \le 2hK + 2 (\frac{2\alpha m}{\beta} + 1) h \sum_{k=2}^K (k-1) \sum_{s, a} \sqrt{\frac{\log (S A (m+1) \pi^2 t_k^3 / 3 \delta)}{2 \max \{1, N_k(s,a)\}}}
	\end{align}
	
	Combining Claim~\ref{thm:pseudoregret} and Lemma~ \ref{lemma:visitcount}, the total pseudo-regret of $K$ episodes of Algorithm~\ref{alg:safeUCRL}
	\begin{align}
	\Delta(T) & = \sum_{k=1}^K \Delta_k \\ 
	& \le 2hK + 2 (\frac{2\alpha m}{\beta} + 1) h \sum_{k=2}^K (k-1) \sum_{s, a} \sqrt{\frac{\log (S A (m+1) \pi^2 t_k^3 / 3 \delta)}{2 \max \{1, N_k(s,a)\}}} \\
	& \le 2hK + 2 (\frac{2\alpha m}{\beta} + 1) hSA \sum_{k=2}^K (k-1) \sqrt{\frac{\log (SA (m+1) \pi^2 t_k^3 / 3 \delta)}{2 (k-1)(\rho h - \sqrt{72\xi \rho h \log(\frac{\varphi  \cdot SAK}{\delta})})}} \\
	& \le 2hK + 2 (\frac{2\alpha m}{\beta} + 1) hSA \sqrt{\log (SA (m+1) \pi^2 T^3 / 3 \delta)} \sum_{k=1}^{K-1} \sqrt{\frac{k}{2(\rho h - \sqrt{72\xi \rho h \log(\frac{\varphi  \cdot SAK}{\delta})})}} \\
	& = 2hK + 2 (\frac{2\alpha m}{\beta} + 1) hSA \sqrt{\frac{\log (SA (m+1) \pi^2 T^3 / 3 \delta)}{2(\rho h - \sqrt{72\xi \rho h \log(\frac{\varphi  \cdot SAK}{\delta})})}} \sum_{k=1}^{K-1} \sqrt{k} \\
	& \le 2hK + 2 (\frac{2\alpha m}{\beta} + 1) hSA \sqrt{\frac{\log (SA (m+1) \pi^2 T^3 / 3 \delta)}{2(\rho h - \sqrt{72\xi \rho h \log(\frac{\varphi  \cdot SAK}{\delta})})}} (K-1) \sqrt{\frac{K}{2}} \\
	& = O(K) + O(K\sqrt{K\log(T/\delta)}) \\
	& \le O(T^{\frac{3}{4}}\sqrt{\log(T/\delta)})
	\end{align}
	
	where the final step follows from $T = \sum_{k=1}^K kh = \frac{K(K-1)}{2} h$, and thus $K < \sqrt{\frac{2T}{h}}$. The second last inequality follows Jensen's inequality. 
\end{proof}

==> intro.tex <==
\section{Introduction}
\label{sec:intro}
Markov Decision Processes (MDPs) have been successfully utilized to model sequential decision-making problems in stochastic environments. In the typical approach to learning a policy, the decision-maker trades off between exploration and exploitation, gradually improving their performance at the task as learning progresses. Reinforcement learning, a standard paradigm of learning in MDPs, has shown exceptional success in a variety of domains such as video games \citep{mnih2015human}, robotics \citep{lillicrap2015continuous, levine2016end}, recommender systems \citep{shani2005mdp}, autonomous vehicles \citep{sallab2017deep}, among many others. 

However, in many of these real-world applications, there is often additional constraints, or specifications that lead to constraints, on the learning problem. 
%For instance, in many applications it is crucial to guarantee  safety while exploring the MDP \citep{amodei2016concrete}---e.g.,  \lily{This is not a good example of "saftey" but rahter just a specification so maybe we can find a safety example a 
For instance, a recommender system should avoid presenting offending items to users and autonomous vehicles must avoid crashing into others while navigating \citep{garcia2015comprehensive} . 
Building algorithms that respect  safety constraints not only during normal operation, but also during the initial learning period, is a question of particular interest \citep{leike2017ai}. This problem is known as the \emph{safe exploration problem} \citep{moldovan2012safe, amodei2016concrete}.
 In the standard MDP framework, an approach for baseline performance is risk-sensitive reinforcement learning \citep{coraluppi1999risk, garcia2015comprehensive}, where the optimization criterion is transformed in order to reflect a subjective measure balancing the return and the risk.

On the other hand, in a safety-critical environment, it is more reasonable to separate the return and the risk criterion, and enforce constraint satisfaction in the learning procedure. A standard formulation for an environment with safety constraints is the constrained MDPs (CMDPs) \citep{altman1999constrained}. A decision-maker facing a  CMDP aims to maximize the total reward while satisfying the constraints on costs in expectation over the whole trajectory. 

In recent literature, policy gradient-based reinforcement learning algorithms have been proposed as a means to learn a policy for a CMDP. The following are two constrained policy search algorithms with state-of-the-art performance guarantees: Lagrangian-based actor-critic algorithm \citep{bhatnagar2012online, chow2018risk} and Constrained Policy Optimization (CPO) \citep{achiam2017constrained}. However, for these policy gradient-based methods, safety is only approximately guaranteed \emph{after} a sufficient learning period. The fundamental issue is that without a model, safety must be learned via trial and error, which means it may be violated during initial learning interactions.

Model-based approaches have utilized Gaussian processes to model the state safety values or the dynamic uncertainties \citep{berkenkamp2017safe, koller2018learning, wachi2018safe, cheng2019end} or utilized Lyapunov-based methods \citep{chow2018lyapunov} to guarantee safety during learning. Although these methods guarantee constraint satisfaction during learning, an arguably valuable analysis of the regret  is lacking.

In this work, we are not only interested in learning the optimal policy that satisfies the constraints via interacting with the stochastic environment, but also in ensuring performance guarantees on the learning algorithm during learning. 
Given that we make the assumption that the rewards and constraint costs are unknown, motivated by upper confidence reinforcement learning (UCRL2) \citep{jaksch2010near}, we introduce the constrained UCRL (C-UCRL) algorithm which combines elements of the classical UCRL2 algorithm with robust linear programming. %\textcolor{red}{this should be in the list of contributions also....}

UCRL2 \citep{jaksch2010near} is an reinforcement learning algorithm that solves MDPs with sub-linear regret. It builds confidence intervals on reward and transition kernel and iteratively solves for policies using value iteration based methods. In contrast to UCRL2 algorithm in standard MDP framework, we study CMDP framework with extra cost criterion. Our approach builds confidence intervals on reward and cost value of state-action pair, considering the transition kernel is taken as known. An example of such CMDP is rover exploration on Mars and the constraint would be to limit the frequency of visiting a potential hazardous state. 
%\textcolor{red}{Need to introduce UCRL since you have not talked about this at all to this point... What is it and what is UCRL2? the reader will be asking these questions. Motivate why we take the UCRL type approach also differentiate our approach from UCRL by remarking that we do not need to learn the transition kernel because its taken as known. this fact also needs to be motivated by an example application... }
We define our goals as follows: (1) maintain constraint satisfaction throughout the learning process with high probability, and (2) achieve sub-linear regret comparing the rewards collected by the algorithm during learning with the reward of an optimal stochastic policy.

%\textcolor{blue}{Maybe in the short version we can skip this bandit part?}
%\lily{Yes, I think this text below can go in a longer version... I think we should hang the longer version on your website so we have time to properly clean it up before it goes on arxiv.}
Of independent interest, out result can also be used in Multi-Armed Bandits (MABs) setting. The MABs problem has been extensively studied in machine learning and statistics as a means to model online sequential decision making. In the classic stochastic MABs setting \citep{auer2002finite}, the decision-maker selects exactly one arm at each round, given the observation of received rewards from arms played in previous round. The goal is to maximize the cumulative reward over a fixed horizon, or equivalently, to minimize regret, which is defined as the difference between the cumulative gain achieved, had the decision-maker always played the best arm, and the realized cumulative gain. Particularly, this setting can be viewed as a MDP problem with only one state and several actions. The analysis of this setting reflects the fundamental tradeoff between the desire to learn better arms (exploration) and the possibility to play arms believed to have high payoff (exploitation).

MABs algorithms have been widely adopted in real applications including recommender systems \citep{li2010contextual}, crowd-sourcing \citep{liu2015online}, real-time bidding problem in ad exchange \citep{chakraborty2010selective} and job finding in labor markets \citep{berry1997bandit}. In reality, taking an action (pulling an arm) is usually inherently costly \citep{ding2013multi}. For instance, in the real-time bidding problem in ad exchange, the bid of an ad is the arm and there is a cost associated with each
pulling of an arm, which is the per-click payment to the ad exchange by the advertiser.

In this work, we study the MABs with budget constraints, such that the per-round costs of the policy in expectation is bounded. Note that our algorithm chooses a randomized policy over all arms instead of selecting exactly one arm at each round. The regret is considered with respect to the optimal policy satisfying the constraints. Our algorithm satisfies budget constraints in each round with high probability and achieves sub-linear regret over finite horizon.

\paragraph{Contributions.} The contributions of this work can be summarized as follows:
\begin{itemize}[itemsep=-5pt, topsep=-10pt]
\item Building on UCLR2, we introduce the C-UCRL algorithm (Algorithm~\ref{alg:safeUCRL}).
    \item We show that C-UCRL is guaranteed to satisfy safety constraints during learning with probability at least $1-\delta$ (Theorem~\ref{thm:deltasafe}) and achieves $ O(T^{\frac{3}{4}}\sqrt{\log(T/\delta)})$ reward regret (Theorem~\ref{thm:regret}); 
    %\textcolor{red}{you probably need to distinguish between regret and reward regret. be clear why you are adding the qualifier 'reward' (i.e. because we have a cost...)}
    \item Of independent interest, the setting we consider subsumes stochastic multi-armed bandits (MABs) with per-round budget constraints, where the optimal policy is a randomized policy across arms. Hence, our results provide novel regret guarantees in this setting as well. 
%\textcolor{red}{are you sure this is novel?} 
\end{itemize}

\paragraph{Organization.}
%\lily{Say we have included a breif overview of related work at the end in some section and longer discussion in the version you will hang on your website.}
The rest of the paper is organized as follows. Section \ref{sec:related_work} list the related work on RL methods solving CMDPs, RL algorithm solving MDPs with regret analysis (UCRL2) as well as MABs algorithms with budget constraint and compare the this paper's contribution to those literature. Mathematical preliminaries and our algorithm are introduced in Section \ref{sec:algo}. Analysis of both constraints satisfaction and reward regret is provided in Section \ref{sec:analysis}.
%Simulations for MABs example and several safety grid world are presented in Section \ref{sec:experiment} to demonstrate the proposed algorithms. Section \ref{sec:conclusion} concludes the paper.
Several illustrative examples which leverage the grid world abstraction are provided in Section \ref{sec:experiment}.
In those experiments we compare our proposed method to Risk-Sensitive UCRL2 algorithm and show that UCRL2 algorithm fails to converge to the optimal policy while our algorithm does.
%\textcolor{red}{Should say here what some of the take aways of the examples are... What do you compare to? and what is the outcome of the comparison...}  
The paper is concluded in Section \ref{sec:conclusion} with a brief summary.





==> oldthreestate.tex <==

\begin{figure}[t]
	\centering
	\subfigure[]{\label{subfig:cmdp}\includegraphics[width=0.3\linewidth]{figure.pdf}} 
	\subfigure[]{\label{subfig:opt_policy}\includegraphics[width=0.4\linewidth]{opt_policy.pdf}}
	\subfigure[]{\label{subfig:lambda}\includegraphics[width=0.19\linewidth]{three_state_lambda.pdf}}
	%\subfigure[Average cost]{\label{subfig:cost}\includegraphics[width=0.3\linewidth]{ave_cost.pdf}}
	%\subfigure[Cumulative regret]{\label{subfig:regret}\includegraphics[width=0.4\linewidth]{cumu_regret.pdf}}
	\caption{Simple CMDP. (a) CMDP structure; (b) optimal policy computed with the true mean reward and mean cost, with and without the constraint on cost, $d=0.2$; (c) probability of constraint violation in 30 training episodes by Risk-Sensitive UCRL2. }%\lily{This example is way too small to be interesting. Can you make it more than 3 states? I think having one toy example is good if it demonstrates somethign interesting like a failure of an alternative or naive algorithm. But beyond that, you need a compellign example that has a large number of states or actions for example... or representing an actual real world problem.}
	\label{fig:cmdp}
\end{figure}

%In this application, autonomous vehicles (agents) explore a region, which can be partitioned into $n$ disjoint subregions (or bins). We can model the system as a CMDP where the states of agents are their bin locations and the actions of a vehicle are defined by the possible transitions to neighboring bins or stay in the current state. Each vehicle collects stochastic rewards and costs while traversing the area.

%Note that the constraints developed in this paper can be interpreted as follows: If the number of vehicles is large where each vehicle is moving according an identical MDP, then the density of vehicles evolves following a Markov Chain and essentially converge to the steady state. Since the physical environment can impose constraints on the number of vehicles in a given state taking a given action, the safety state constraints can be imposed to bound the expected number of vehicles at steady state.

To  demonstrate the performance of C-UCRL, we start with a simple three state CMDP. As show in Figure \ref{subfig:cmdp}, the CMDP we consider has three states and two action. An agent can take either a \emph{risky} exploratory action in which the navigate to another state or they can take the \emph{safe} action and remain in the current state.
 There is no reward or cost for staying in the current state but there will be a stochastic reward and cost if the agent navigates. In the simulation, the reward and cost of each state-action pair are each draw from a binomial distribution, with the means defined in the labels on edges in Figure~\ref{subfig:cmdp}.  Obviously, without this constraint, the optimal policy is to navigate in each of the states. In this problem, we consider the constraint that in expectation, the average cost should be less than $0.2$. This constraint prevents the agents from continuously navigating between the three states. In particular, as shown in Figure~\ref{subfig:opt_policy}, the constrained optimal policy is a randomized policy that has positive probability on the safe action in each state. The relatively conservative baseline policy we use in C-UCRL for exploration is staying in the current state with probability $0.8$ and navigate to the next state with probability $0.2$. 

\begin{figure}[t]
	\centering
		\subfigure[]{\label{fig:regret_cost}\includegraphics[width=0.475\linewidth]{three_states.pdf}}\subfigure[]{\label{fig:policy}\includegraphics[width=0.525\linewidth]{three_state_policy.pdf}}
	\caption{C-UCRL vs.~Risk-Sensitive UCRL2: (a) Cumulative regret and average cost for C-UCRL and risk sensitive UCRL2; (b) Policy learned by C-UCRL and risk sensitive UCRL2.}
\end{figure}

We compare our approach with the UCRL2 algorithm. However, UCRL2 does not allow for constraints or multiple reward/cost criteria. Hence,  we leverage the idea of risk sensitive reinforcement learning \citep{leike2017ai}, where we treat a linear combination of reward and cost---i.e., $r - \lambda c$---as the reward for the UCRL2 algorithm. The hyperparameter $\lambda$ represents the trade off between the reward and cost. Figure \ref{subfig:lambda} shows the constraint violation probability in 30 training episodes by UCRL2 algorithm with different $\lambda$. Figure \ref{fig:regret_cost} shows the cumulative regret and average cost of the C-UCRL and UCRL2 algorithms. As we can see,  when the cost value is underestimated ($\lambda = 1.9$), applying UCRL2 directly leads to a `good' reward (i.e., the regret is negative as it gets more reward than the optimal randomized policy), yet the constraints are violated.  On the other hand, when the costs are overestimated ($\lambda = 2.1$), UCRL2 is too conservative about the cost and, thus, receives high regret. We can observe that C-UCRL doesn't violate the constraint during learning. In this experiment, $\delta$ is set to be $0.1$, meaning that with probability at least $0.9$, the constraint will not be violated in all episodes.
%\textcolor{red}{What happens if you put $\lambda=2$? or somewhere in between? can you get the same performance? Seems like you need to do more of a sweep here over lambda to see what happens. Picking two values seems like a gross over simplification. Also you need to highlight what the take away is. Is it is simply that UCRL2 will always lead to a constraint violation? What is $\delta$ for our problem here? and how often do we actually violate the constraint?}
%\begin{figure}[t]
%	\centering
%	\includegraphics[width=0.9\linewidth]{three_state_policy.pdf}
%	\caption{Policy learned by C-UCRL and risk sensitive UCRL2.}
%	\label{fig:policy}
%\end{figure}

The fundamental problem with UCRL2 is that with only one criterion, the policy it learns will always be a deterministic policy, while in this constrained MDP, the optimal policy is randomized.  %\textcolor{red}{This is only true with high probability what is $\delta$ for this example?} 
Figure \ref{fig:policy} shows the policy learned by C-UCRL and risk-sensitive UCRL2. When $\lambda = 1.9$, UCRL2 learn the optimal policy as there is no constraint, which leads to constraint violation. When $\lambda=2.1$, the policy learned by UCRL2 is to stay in one state forever. On the contrary, the policy learned by C-UCRL algorithm converges to the optimal randomized policy.
%\textcolor{red}{This is sort of repetitive. you should combine this paragraph and the one above. This paragraph is actually better though my questions above still stand. }
%C-UCRL is able to learn a randomized policy that guarantees constraint satisfaction and achieve sub-linear regret.
%Also note that UCRL algorithm tend to be less stable while learn because to have a good balancing between reward and cost, $\lambda$ is chosen such that in expectation, $r - \lambda c$ is close to zero. As shown in the figure, this will make the policy during learning tend to be unstable.

==> preliminary_old.tex <==
%\section{Constrained Upper Confidence Reinforcement Learning Algorithm}
%\label{sec:algo}

% One motivation example is taxi navigating in the city. \lily{This doesn't make sense. above you say the transition kernel is known but below you say it is unknow for the taxi example: "which is considerably static and unknown"... And the dynamics would not be the city map. The interconnection structure would be the city map, but whether a driver traverses an edge depends on their actions and where their fare wants to go, so its not clear to me why this is an example where the transition kernel is known. So this paragraph needs to be revised. Find an example where it makes sense that you know the transition kernel and where it is stochastic. Maybe you can say that in the taxi case that the transition kernel is determined by the map structure, the actions of the driver (which typically are dictated by something like google maps once they have a fare), and the demand for taxis at nodes. And as such it is reasonable that this P could be estimated... this is still a bit of a stretch to me... Also you haven't introduced the notation for P yet. This paragraph should come after the paragraph below} The transition dynamic is the city map, which is considerably static and unknown but the profit and fuel consumption depend on several factors such as weather, are relatively stochastic and unknown.

An MDP is a tuple $(\mathcal{S}, \mathcal{A}, P, r)$, where $\mathcal{S}$ is the set of states, $\mathcal{A}$ is the set of actions, $P: \mathcal{S} \times \mathcal{A} \times \mathcal{A} \rightarrow [0,1]$ is the transition kernel such that $P(s'|s,a)$ is the probability of transitioning to state $s'$ given that the previous state was $s$ and the agent took action $a$ in $s$, and $r: \mathcal{S} \times \mathcal{A} \rightarrow [0,1]$ is the reward function. A stationary policy $\pi: \mathcal{S} \times \mathcal{A} \rightarrow [0,1]$ is a map from states to a probability distribution over actions, with $\pi(a|s)$ denoting the probability of selecting action $a$ in state $s$. We consider the setting that the transition kernel $P(s'|s,a)$ is known to the agent, but the reward and costs are stochastic and unknown. In the example of rover exploration on Mars, the controlling is aware of the transition probability of next state based on its action, but safety values of each state are unknown.
%\textcolor{red}{Some example where this is true in practice?}
Let $S = |\mathcal{S}|$ and $A = |\mathcal{A}|$ where $|\cdot|$ is the cardinality of its argument. We use the notation $[\cdot]=\{1,\ldots, \cdot\}$ for index sets.

A CMDP is an MDP augmented with `cost' constraints that restrict the set of allowable policies for that MDP. 
For a given CMDP, we consider the performance measure to be the \emph{infinite horizon average reward} which is given by
\begin{equation}
J(\pi) =\textstyle \lim_{T \to \infty} \mathbb{E}_{\tau \sim \pi} \big[ \frac{1}{T} \sum_{t=0}^{T-1} r(s_t, a_t) \big]
\end{equation}
where $\tau$ denotes a trajectory $\tau = (s_0, a_0, s_1, \dots)$, and $\tau \sim \pi$ is shorthand for indicating that the distribution over trajectories depends on $\pi$: $s_0 \sim p(s_0), a_t \sim \pi(\cdot|s_t), s_{t+1} \sim P(\cdot|s_t, a_t)$. Similarly, define the \emph{average constraint costs} by
\begin{equation}
C_i(\pi) = \textstyle\lim_{T \to \infty} \mathbb{E}_{\tau \sim \pi} \big[ \frac{1}{T} \sum_{t=0}^{T-1} c_i(s_t, a_t) \big].
\end{equation}
where $\{c_1, \dots, c_m\}$ with $c_i: \mathcal{S} \times \mathcal{A} \rightarrow [0,1]$ are the cost constraints. 
The CMDP is then defined by
% that solves
\begin{equation}
\max_{\pi} \ \{J(\pi)|\  C_i(\pi) \le d_i, \ \ \forall\ i \in [m]\}
\end{equation}
where $\{d_1, \ldots, d_m\}$ are upper bounds on the average constraint costs.  Note that without loss of generality both reward and cost functions are random variables with a distribution supported on $[0,1]$.

Denote the mean of reward and cost constraint functions as $\bar{r}(s, a) = \mathbb{E}[r(s,a)]$, $\bar{c}_i = \mathbb{E}[c_i(s,a)]$ where the expectation is taken with respect to the distribution of the reward and cost function of that state-action pair $(s,a)$.

%\lily{We may be able to put this expanded LP in the longer version and just write out the matrix form.}
If the transition kernel $P(s'|s,a)$, the mean of the reward function $\bar{r}(s, a)$, and mean cost functions $\bar{c}_i(s,a)$ are all given, them we can solve the CMDP by solving the following linear program \citep{altman1999constrained}:
\begin{align}
\max_{y} & \quad \textstyle\sum_{s, a} \bar{r}(s, a) y(s, a) \\
\text{s.t.} & \textstyle\quad \sum_{a'} y(s', a') = \sum_{s, a} P(s'|s, a) y(s, a) \\
& \quad \textstyle\sum_{s, a} y(s, a) = 1, \quad y(s, a) \ge 0 \\
& \quad \textstyle\sum_{s, a} \bar{c}_i(s, a) y(s, a) \le d_i, \ i\in [m]
\end{align}
which can also be written in matrix form:
\begin{equation}
\max_{y} \{ \  \bar{r}^\top y \ |\  I_o y = P y, \  \mathbf{1}^\top y = 1,\  y \ge 0, \ \bar{c}^\top y \le d\}
\end{equation}
where $\bar{r} \in \mathbb{R}^{SA}, y \in \mathbb{R}^{SA}$, $\bar{c} \in \mathbb{R}^{SA\times m}, d \in \mathbb{R}^m$, $P \in \mathbb{R}^{S \times SA}$, and  $I_o \in \mathbb{R}^{S \times SA}$ is a sparse matrix built by placing $S$ row blocks of length $A$ in a block diagonal fashion, where each row block consists of all ones. 

Here, $y \in \mathbb{R}^{S \times A}$ represents the steady-state occupation measure and is defined by
\begin{equation}
y(s, a) = \textstyle\lim_{T \to \infty} \mathbb{E}_{\tau \sim \pi} \big[\frac{1}{T} \sum_{t=0}^{T-1} \mathbf{1} \{ s_t=s, a_t=a \} \big].
\end{equation}
With $\bar{y}$ the solution of this linear program, the optimal  stationary policy is
\begin{equation}
\bar{\pi}(a|s) = \textstyle\bar{y}(s, a)/(\sum_{a \in \mathcal{A}} \bar{y}(s, a)).
\end{equation}

It is worth noting that unlike in tabular MDPs without constraints, where the optimal policy is always deterministic, the optimal policy in CMDPs could be stochastic \citep{puterman2014markov}.  It is, in fact, trivial to solve the CMDP if the optimal policy in CMDPs is deterministic because that means the constraints are not active.

